Multipole Moments of Double Heavy $J^P = \frac{3}{2}^+$ Baryons

In the present study, we calculate the multipole moments of spin-3/2 doubly heavy baryons within the light cone QCD sum rules. We compare our results on magnetic dipole moments with results existing in the literature. The results obtained in the present work may be useful for a deeper understanding of the properties of doubly heavy baryons as well as in the analysis of their strong and electromagnetic decays.

==> ref.tex <==
\bibliographystyle{ieeetr}
\bibliography{ref}
